Representations as Language: An Information-Theoretic Framework for Interpretability

Large scale neural models show impressive performance across a wide array of linguistic tasks. Despite this they remain, largely, black-boxes - inducing vector-representations of their input that prove difficult to interpret. This limits our ability to understand what they learn, and when the learn it, or describe what kinds of representations generalise well out of distribution. To address this we introduce a novel approach to interpretability that looks at the mapping a model learns from sentences to representations as a kind of language in its own right. In doing so we introduce a set of information-theoretic measures that quantify how structured a model's representations are with respect to its input, and when during training that structure arises. Our measures are fast to compute, grounded in linguistic theory, and can predict which models will generalise best based on their representations. We use these measures to describe two distinct phases of training a transformer: an initial phase of in-distribution learning which reduces task loss, then a second stage where representations becoming robust to noise. Generalisation performance begins to increase during this second phase, drawing a link between generalisation and robustness to noise. Finally we look at how model size affects the structure of the representational space, showing that larger models ultimately compress their representations more than their smaller counterparts.

==> citation_notes.tex <==




\section{Formalities, Footnotes, and Floats}

Use standard APA citation format. Citations within the text should
include the author's last name and year. If the authors' names are
included in the sentence, place only the year in parentheses, as in
\citeA{NewellSimon1972a}, but otherwise place the entire reference in
parentheses with the authors and year separated by a comma
\cite{NewellSimon1972a}. List multiple references alphabetically and
separate them by semicolons
\cite{ChalnickBillman1988a,NewellSimon1972a}. Use the
``et~al.'' construction only after listing all the authors to a
publication in an earlier reference and for citations with four or
more authors.


\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first
footnote.} in the text. Place the footnotes in 9~point font at the
bottom of the column on which they appear. Precede the footnote block
with a horizontal rule.\footnote{Sample of the second footnote.}


\subsection{Tables}

Number tables consecutively. Place the table number and title (in
10~point) above the table with one line space above the caption and
one line space below it, as in Table~\ref{sample-table}. You may float
tables to the top or bottom of a column, and you may set wide tables across
both columns.

\begin{table}[H]
\begin{center} 
\caption{Sample table title.} 
\label{sample-table} 
\vskip 0.12in
\begin{tabular}{ll} 
\hline
Error type    &  Example \\
\hline
Take smaller        &   63 - 44 = 21 \\
Always borrow~~~~   &   96 - 42 = 34 \\
0 - N = N           &   70 - 47 = 37 \\
0 - N = 0           &   70 - 47 = 30 \\
\hline
\end{tabular} 
\end{center} 
\end{table}


\subsection{Figures}

All artwork must be very dark for purposes of reproduction and should
not be hand drawn. Number figures sequentially, placing the figure
number and caption, in 10~point, after the figure with one line space
above the caption and one line space below it, as in
Figure~\ref{sample-figure}. If necessary, leave extra white space at
the bottom of the page to avoid splitting the figure and figure
caption. You may float figures to the top or bottom of a column, and
you may set wide figures across both columns.

\begin{figure}[H]
\begin{center}
\fbox{CoGNiTiVe ScIeNcE}
\end{center}
\caption{This is a figure.} 
\label{sample-figure}
\end{figure}


\section{Acknowledgments}

In the \textbf{initial submission}, please \textbf{do not include
  acknowledgements}, to preserve anonymity.  In the \textbf{final submission},
place acknowledgments (including funding information) in a section \textbf{at
the end of the paper}.


\section{References Instructions}

Follow the APA Publication Manual for citation format, both within the
text and in the reference list, with the following exceptions: (a) do
not cite the page numbers of any book, including chapters in edited
volumes; (b) use the same format for unpublished references as for
published ones. Alphabetize references by the surnames of the authors,
with single author entries preceding multiple author entries. Order
references by the same authors by the year of publication, with the
earliest first.

Use a first level section heading, ``{\bf References}'', as shown
below. Use a hanging indent style, with the first line of the
reference flush against the left margin and subsequent lines indented
by 1/8~inch. Below are example references for a conference paper, book
chapter, journal article, dissertation, book, technical report, and
edited volume, respectively.

\nocite{ChalnickBillman1988a}
\nocite{Feigenbaum1963a}
\nocite{Hill1983a}
\nocite{OhlssonLangley1985a}
% \nocite{Lewis1978a}
\nocite{Matlock2001}
\nocite{NewellSimon1972a}
\nocite{ShragerLangley1990a}


==> tables/flip_table.tex <==
\begin{table}[ht]

  %\caption{Your Table Caption}

  \begin{tabularx}{\linewidth}{lrrrrrrrr}                        

    \toprule
     & \multicolumn{2}{r}{Alignment} & \multicolumn{2}{r}{Contextualisation} & \multicolumn{2}{r}{Disentanglement} & \multicolumn{2}{r}{Information H(Y)} \\
     & \multicolumn{2}{r}{I(pos,Y)} & \multicolumn{2}{r}{H(Y|pos)} & \multicolumn{2}{r}{H(Y)-H(Y|-pos)} & \multicolumn{2}{r}{H(Y)} \\
     & mean & z & mean & z & mean & z & mean & z \\
    condition &  &  &  &  &  &  &  &  \\
    \midrule
    large & 0.340696 & 0.008691 & 0.887997 & 0.001737 & 0.016871 & 0.000431 & 0.927506 & 0.001174 \\
    medium & 0.375028 & 0.008128 & 0.890199 & 0.001074 & 0.017098 & 0.000280 & 0.932894 & 0.000835 \\
    small & 0.423337 & 0.012142 & 0.888463 & 0.001545 & 0.018537 & 0.000503 & 0.936802 & 0.000658 \\
    \bottomrule
  \end{tabularx}
\end{table}

\begin{table}[ht]

  %\caption{Your Table Caption}

  \begin{tabularx}{\linewidth}{lrrrrrrrr}                        

    \textbf{SLOG} & \multicolumn{2}{c}{\small{small}} & \multicolumn{2}{c}{\small{medium}} & \multicolumn{2}{c}{\small{large}} \\
    \midrule
    \small{Information} & \acc{1.4095}{5} & \acc{2.5}{1.4}& \acc{1.4095}{1.4}\\
    \small{Contextualisation} & \acc{1.4095}{5} & \acc{2.5}{1.4}& \acc{1.4095}{1.4}\\
    \small{Disentanglement} & \acc{1.4095}{5} & \acc{2.5}{1.4}& \acc{1.4095}{1.4}\\
    \small{Alignment}  & \acc{1.4095}{5} & \acc{2.5}{1.4}& \acc{1.4095}{1.4}\\
    \small{Accuracy} & \acc{1.4095}{5} & \acc{2.5}{1.4}& \acc{1.4095}{1.4}\\


    \midrule
    \multicolumn{7}{l}{\textbf{CFQ}} \\
    \midrule
    \small{Information} & \acc{1.4095}{5} & \acc{2.5}{1.4}& \acc{1.4095}{1.4}\\
    \small{Contextualisation} & \acc{1.4095}{5} & \acc{2.5}{1.4}& \acc{1.4095}{1.4}\\
    \small{Disentanglement} & \acc{1.4095}{5} & \acc{2.5}{1.4}& \acc{1.4095}{1.4}\\
    \small{Alignment} & \acc{1.4095}{5} & \acc{2.5}{1.4}& \acc{1.4095}{1.4}\\
    \small{Accuracy} & \acc{1.4095}{5} & \acc{2.5}{1.4}& \acc{1.4095}{1.4}\\

    \bottomrule
  \end{tabularx}
\end{table}


==> tables/table.tex <==

\begin{table}[ht]

  %\caption{Your Table Caption}

  \begin{tabularx}{\linewidth}{>{\hsize=0.7\hsize}l
                              >{\hsize=0.05\hsize}c
                              >{\hsize=0.05\hsize}c
                              >{\hsize=0.05\hsize}c
                              >{\hsize=0.05\hsize}c
                              >{\hsize=0.05\hsize}c
                              >{\hsize=0.05\hsize}c}                        
\hline
    \textbf{SLOG} & \multicolumn{2}{c}{small} & \multicolumn{2}{c}{medium} & \multicolumn{2}{c}{large} \\
    \midrule
    \small{Information} \tiny{H(Y)}& \acc{1.4095}{5} & \acc{2.5}{1.4}& \acc{1.4095}{1.4}\\
    \small{Contextualisation \tiny{H(Y|token)}} & \acc{1.4095}{5} & \acc{2.5}{1.4}& \acc{1.4095}{1.4}\\
    \small{Disentanglement} \tiny{H(Y)-H(Y$|\neg token$)} & \acc{1.4095}{5} & \acc{2.5}{1.4}& \acc{1.4095}{1.4}\\
    \small{Alignment} \tiny{I(X,Y)} & \acc{1.4095}{5} & \acc{2.5}{1.4}& \acc{1.4095}{1.4}\\
    \small{Accuracy} & \acc{1.4095}{5} & \acc{2.5}{1.4}& \acc{1.4095}{1.4}\\


    \midrule
    \multicolumn{7}{l}{\textbf{CFQ}} \\
    \midrule
    \small{Information} \tiny{H(Y)}& \acc{1.4095}{5} & \acc{2.5}{1.4}& \acc{1.4095}{1.4}\\
    \small{Contextualisation \tiny{H(Y|token)}} & \acc{1.4095}{5} & \acc{2.5}{1.4}& \acc{1.4095}{1.4}\\
    \small{Disentanglement} \tiny{H(Y)-H(Y$|\neg token$)} & \acc{1.4095}{5} & \acc{2.5}{1.4}& \acc{1.4095}{1.4}\\
    \small{Alignment} \tiny{I(X,Y)} & \acc{1.4095}{5} & \acc{2.5}{1.4}& \acc{1.4095}{1.4}\\
    \small{Accuracy} & \acc{1.4095}{5} & \acc{2.5}{1.4}& \acc{1.4095}{1.4}\\

    \bottomrule
  \end{tabularx}
\end{table}
